CP-Guard: Malicious Agent Detection and Defense in Collaborative Bird's Eye View Perception

Collaborative Perception (CP) has shown a promising technique for autonomous driving, where multiple connected and autonomous vehicles (CAVs) share their perception information to enhance the overall perception performance and expand the perception range. However, in CP, ego CAV needs to receive messages from its collaborators, which makes it easy to be attacked by malicious agents. For example, a malicious agent can send harmful information to the ego CAV to mislead it. To address this critical issue, we propose a novel method, CP-Guard, a tailored defense mechanism for CP that can be deployed by each agent to accurately detect and eliminate malicious agents in its collaboration network. Our key idea is to enable CP to reach a consensus rather than a conflict against the ego CAV's perception results. Based on this idea, we first develop a probability-agnostic sample consensus (PASAC) method to effectively sample a subset of the collaborators and verify the consensus without prior probabilities of malicious agents. Furthermore, we define a collaborative consistency loss (CCLoss) to capture the discrepancy between the ego CAV and its collaborators, which is used as a verification criterion for consensus. Finally, we conduct extensive experiments in collaborative bird's eye view (BEV) tasks and our results demonstrate the effectiveness of our CP-Guard. Code is available at https://github.com/CP-Security/CP-Guard

==> sections/checklist.tex <==
\section{Reproducibility Checklist}

This paper:

\begin{checkboxlist}
    \item [\done] Includes a conceptual outline and/or pseudocode description of AI methods introduced 
    \item [\done] Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results 
    \item [\done] Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper 
\end{checkboxlist}


% \begin{checkboxlist}
% \item 
\ 


\noindent Does this paper make theoretical contributions? (Yes)
\begin{checkboxlist}
    \item [\done] All assumptions and restrictions are stated clearly and formally. 
    \item [\done] All novel claims are stated formally (e.g., in theorem statements). 
    \item [\done] Proofs of all novel claims are included. 
    \item [\done]Proof sketches or intuitions are given for complex and/or novel results. 
    \item [\done] Appropriate citations to theoretical tools used are given. 
    \item [\done] All theoretical claims are demonstrated empirically to hold. 
    \item [\done] All experimental code used to eliminate or disprove claims is included. 
\end{checkboxlist}
% \end{checkboxlist}

\ 


\noindent Does this paper rely on one or more datasets? (Yes)
\begin{checkboxlist}
    \item[\done]  A motivation is given for why the experiments are conducted on the selected datasets 
    \item[\wontfix] All novel datasets introduced in this paper are included in a data appendix. 
    \item[\done] All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. 
    \item[\done] All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. 
    \item[\done] All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. 
    \item[\done] All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. 
\end{checkboxlist}


\ 


\noindent Does this paper include computational experiments? (Yes)

\begin{checkboxlist}
    \item [\wontfix] Any code required for pre-processing data is included in the appendix.
    \item [\wontfix] All source code required for conducting and analyzing the experiments is included in a code appendix. 
    \item [\done] All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. 
    \item [\done] All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from 
    \item [\done] If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. 
    \item [\done] This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. 
    \item [\done] This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. 
    \item [\done] This paper states the number of algorithm runs used to compute each reported result. 
    \item [\done] Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. 
    \item [\done] The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). 
    \item [\done] This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. 
    \item [\done] This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. 
\end{checkboxlist}


